KML: Using Machine Learning to Improve Storage Systems

Operating systems include many heuristic algorithms designed to improve overall storage performance and throughput. Because such heuristics cannot work well for all conditions and workloads, system designers resorted to exposing numerous tunable parameters to users -- thus burdening users with continually optimizing their own storage systems and applications. Storage systems are usually responsible for most latency in I/O-heavy applications, so even a small latency improvement can be significant. Machine learning (ML) techniques promise to learn patterns, generalize from them, and enable optimal solutions that adapt to changing workloads. We propose that ML solutions become a first-class component in OSs and replace manual heuristics to optimize storage systems dynamically. In this paper, we describe our proposed ML architecture, called KML. We developed a prototype KML architecture and applied it to two case studies: optimizing readahead and NFS read-size values. Our experiments show that KML consumes less than 4KB of dynamic kernel memory, has a CPU overhead smaller than 0.2%, and yet can learn patterns and improve I/O throughput by as much as 2.3x and 15x for two case studies -- even for complex, never-seen-before, concurrently running mixed workloads on different storage devices.

==> background.tex <==
\section{Background and Motivation}
\label{sec:background}

\ezk{move 1-2 sentences from here to intro, say about paradigm, rest
  can be removed.  remove all background.tex file.}

% Topic 1: How OS can benefit from this what is our vision? stage 1
%          tune stage 2 complete algorithm
% Topic 2: Concerns about ML - transparency, predictability

We discuss how ML can benefit storage systems and address potential
concerns regarding integrating ML into storage systems and OSs.

\ezk{Problem 1: at end of intro, you said this section would be
  ``brief ML background'' -- the reader expects a small tutorial.  Do
  we even need a tutorial, given that we hope the reviewer will
  already understand enough ML?  Worse, this section title is not just
  ``background'' but also ``motivation'' -- there's a disconnect b/t
  what you PROMISED and what you DELIVERED.}

\ezk{Problem 2: the ``vision'' pgf below is NOT an ML tutorial, You
  just rehash what we did, again calling too much attention to the 2
  use cases: you already mentioned the 2 in intro, and you'll be
  covering them again in much more depth later on.  So most of the
  ``vision'' text seems duplicative and wastes space.  Maybe we can
  cut much of it and save the space?  We can import a couple of
  sentences in ``vision'' into the intro and be done, I think.}

%----------------------------------------------------------------------
\paragraph{Our vision}
%
\kml is designed to replace OS-level storage system heuristics and
system parameter tuning.  Thus, a \kml application first
observes the target component by collecting data from probes that
are placed in the kernel.  The data collected is
used to train an ML model using \kml's functionality APIs.
The \kml application  then use the model to predict and tune system
parameters.
%
Our use cases follow the \emph{observe-and-tune} paradigm to reduce
overhead introduced by the ML models.
%
\ezk{I don't see the connection b/t the prev and next sentences: what
  does observe/tune have to do with low overheads?}
%
Therefore, we do not impose extra overheads on storage
components that require low latency and predictable performance.
%
The two \kml use-cases that we detail in this paper are ML models
developed (1) to tune readahead sizes on a per-disk and per-file basis
and (2) to tune NFS \stt{rsize} value.  We chose these two examples
because:
%
\begin{inparaenum}[(i)]
%
\item their storage components can significantly benefit from
  fine-tuned parameters,
%
\item they require adaptation to a variety of different workloads, which is crucial in providing
  optimal performance, and
%
\item it proves that adding asynchronous ML computation (see
  Section~\ref{sec:eval:kml}) will \emph{not} negatively impact
  critical I/O paths.
%
\end{inparaenum}

%\ezk{flow from before to next pgf is a bit odd}
%\umit{agreed we already mentioned this in intro and related work, commented out}
%\andrew{It's not clear to me what is meant by "We implemented an
%observe-and-tune paradigm to reduce overheads introduced by the ML
%models." what alternative paradigms could we have chosen to
%implement? why do they have higher overheads? are you saying that we
%chose this over, for example, reinforcement learning because of lower
%overhead?}
%\umit{we chose this over inline predictions not RL. RL is just a type
%of ML.}
%
%There is a growing trend for using ML to optimize caching
%algorithms~\cite{shi2019applying, hashemi-corr18-learning} and data
%structures~\cite{kraska2018case}.  In the future, we plan to use \kml
%to build entire OS level storage components or algorithms using ML
%methods such as page cache replacement and directory cache.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% For Emacs:
% Local variables:
% fill-column: 70
% End:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% For vim:
% vim:textwidth=70
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LocalWords:  overviewing readahead ra explainability rsize


==> fig-data-collection.tex <==
\begin{figure}[thbp]
  \centering
  \includegraphics[width=1.0\columnwidth]{figures/graphs/data-collection-histogram}
  \caption{Distribution of total data collection overhead
    (milliseconds) in every second when \stt{readseq} and
    \stt{mixgraph} workloads are running.}
  \label{fig:data-collection-overhead}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% For Emacs:
% Local variables:
% fill-column: 70
% End:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% For vim:
% vim:textwidth=70
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LocalWords:  readahead NVMe RocksDB readrandom readsequential mis
% LocalWords:  readrandomwriterandom readreverse mixgraph readseq


==> tab-api.tex <==
% all-metrics summary table

\begin{table}[ht]
\centering
\begin{Verbatim}[fontsize=\footnotesize,fontfamily=lmss,commandchars=\\\{\}]

\textcolor{blue}{loss} *\textcolor{darkgreen}{build_loss}(\textcolor{blue}{void} *internal, \textcolor{blue}{loss_type} type);
\textcolor{blue}{void} \textcolor{darkgreen}{add_layer}(\textcolor{blue}{layers} *existing_layers, \textcolor{blue}{layer} *new_layer);
\textcolor{blue}{void} \textcolor{darkgreen}{create_async_thread}(\textcolor{blue}{model_multithreading} *multithreading,
        \textcolor{blue}{model_data} *data, \textcolor{blue}{kml_thread_func} func, \textcolor{blue}{void} *param);
\textcolor{blue}{sgd_optimizer} *\textcolor{darkgreen}{build_sgd_optimizer}(\textcolor{blue}{float} learning_rate,
        \textcolor{blue}{float} momentum, \textcolor{blue}{layers} *layer_list, \textcolor{blue}{loss} *loss);
\end{Verbatim}
\caption{\kml API examples}
\label{tab:api-table}
\end{table}

% \ezk{I don't know how much Table \ref{tab:api-table} really helps us.
%   We don't really describe it, we don't say why we have THESE specific
%   functions, and whether we tried different APIs.  It's only 4
%   examples out of over 30 as you say.  Does it really matter what the
%   API actually is, when the main goal is to say that we have the same
%   API in user+kernel?  Maybe we should just say ``for brevity, the
%   full API is not described here, but our full code is already
%   released''?}
% \umit{agreed and fixed in next paragraph, we can remove this table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% For Emacs:
% Local variables:
% fill-column: 70
% End:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% For vim:
% vim:textwidth=70
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% LocalWords:  readahead NVMe mixgraph multithreading kml func param
% LocalWords:  sgd darkgreen

